Improving Energy Saving of One-sided Matrix Decompositions on CPU-GPU Heterogeneous Systems

One-sided dense matrix decompositions (e.g., Cholesky, LU, and QR) are the key components in scientific computing in many different fields. Although their design has been highly optimized for modern processors, they still consume a considerable amount of energy. As CPU-GPU heterogeneous systems are commonly used for matrix decompositions, in this work, we aim to further improve the energy saving of one-sided matrix decompositions on CPU-GPU heterogeneous systems. We first build an Algorithm-Based Fault Tolerance protected overclocking technique (ABFT-OC) to enable us to exploit reliable overclocking for key matrix decomposition operations. Then, we design an energy-saving matrix decomposition framework, Bi-directional Slack Reclamation(BSR), that can intelligently combine the capability provided by ABFT-OC and DVFS to maximize energy saving and maintain performance and reliability. Experiments show that BSR is able to save up to 11.7% more energy compared with the current best energy saving optimization approach with no performance degradation and up to 14.1% Energy * Delay^2 reduction. Also, BSR enables the Pareto efficient performance-energy trade-off, which is able to provide up to 1.43x performance improvement without costing extra energy.

==> abft.tex <==
\subsection{Determine Suitable Clock Frequencies}
\label{abft}
To handle soft error, we choose to use ABFT since it brings much lower fault tolerance overhead compared with more general application level duplication based approaches such as DMR (100\% overhead) or TMR (200\% overhead). ABFT is an application-specific approach and it is usually designed for matrix operations including matrix decompositions focused in this work. It is based on the idea that if we encode certain amount of matrix information in checksums before a matrix operation and apply the same matrix operation also to checksums, the checksum relation would still hold for the result matrix. By verifying the checksum relations, we are able to detect or even correct errors in the result matrix. 

Depending on how much information is encoded in checksums, the error tolerance strength is different. Currently, there are two commonly ways to do checksum encoding (i.e., checksum scheme). (1) Single side checksum scheme encodes matrices along either rows or columns (i.e., calculate the sum of elements of every row or column). Since it only encode matrix in one dimension, it brings relative lower overhead. However, it can only efficiently tolerate 0D error pattern.  (2) Full checksum scheme encodes matrices along both rows and column at the same time. Since it encode matrices in both dimensions, it brings stronger protection i.e., both 0D and 1D error pattern. However, it also brings higher fault tolerance overhead. 


Since there is a limitation on how many error it can correct for a certain checksum design and the number of errors can increase with the raising of processor clock frequency, it is important that we determine clock frequencies and checksum designs that can ensure all errors can be detected and corrected with a high confidence. Otherwise, undetected or uncorrected error would cause serious error propagation later, which requires recovery with high overhead. In this work, we find that it is useful to estimate the max possible processor clock frequencies given two checksum designs. In order to do that, we first define a error rate function $R$ given clock frequency that can be derived from \textbf{Fig. \ref{tmu-error-rate} - \ref{pd-error-rate}}:

$$\lambda_{f, error\_type} = R(f, error\_type)$$



where $\lambda$ is the error rate of a certain $error\_type$. The $error\_type$ can be 0D, 1D, or 2D. $f$ is the processor clock frequency. Assuming the rate is constant for a given clock frequency, we can treat the distribution of probability errors occur during a period of time as Poisson distribution. So, we can calculate the probability of have error less or equal than $k$ during a period of time $T$ using the CDF of Poisson distribution function:

\begin{align}
\label{cdf}
P (\#\ of\ errors\ in\ error\_type \leqslant  k) &=& \\ \nonumber
 \sum_{i=0}^{k}\frac{e^{-\lambda_{f, error\_type}T} (\lambda_{f, error\_type} T)^{i}}{i!}
\end{align}

Based on equation \ref{cdf}, we can define a function $F$ that outputs the max possible clock frequency that leads to less to equal to $k$ errors $error\_type$ during time period of $T$ with at least probability of $p$:

$$f_{max} = F(k, error\_type, T, p)$$


For single side checksum, it can only tolerate up to one 0D error propagation. Since we are encoding checksum for each $nb\times nb$ matrix block individually, it can tolerate up to $\frac{m}{nb} \times \frac{n}{nb}$ 0D error propagations for matrix size of $m \times n$. However, it cannot tolerate any 1D or 2D error propagations. 


So, the max possible clock frequency is estimated as:
\begin{align}
f_{max\_single} = min(F(\frac{m}{nb} \times \frac{n}{nb}, 0D, T_{OP}, p_0), \\ F(0, 1D, T_{OP}, p_1), F(0, 2D, T_{OP}, p_2))
\end{align}

Similarly, we can also estimate the max possible clock frequency for full checksum as:

\begin{align}
f_{max\_full} = min(F(\frac{m}{nb} \times \frac{n}{nb}, 0D, T_{OP}, p_0), \\ F(\frac{m}{nb} \times \frac{n}{nb}, 1D, T_{OP}, p_1), \\ F(0, 2D, T_{OP}, p_2))
\end{align}

where $T_{OP}$ is the execution time of this matrix operation, which can be obtained from our algorithmic prediction model. $p_0, p_1, p_2$ can be set as desired. Higher probabilities such as 99\% indicate that from 99\% of the case ABFT can handle all errors. However, higher probabilities also impose a stricter rule on clock frequency adjustment, which brings a trade-off here.




==> gap.tex <==
\section{Energy consumption gap}
Before we optimize the energy consumption of matrix decompositions, it is necessary to first know the lowest achievable energy consumption of the state-of-the-art energy-saving optimized matrix decompositions, 
as well as the theoretical minimum energy consumption given the same workload.
It is important for us to understand the gap between the two.
We define theoretical minimum energy consumption as follows:
$$E_{theoretical\_min} = \frac{W^{CPU}_{total}}{K^{CPU}_{max}} + \frac{W^{GPU}_{total}}{K^{GPU}_{max}}$$
where $W^{CPU/GPU}_{total}$ is the total amount of workload assigned to CPU or GPU and $K^{CPU/GPU}_{max}$ is the maximum achievable energy efficiency of CPU or GPU.
As shown in \textbf{Figure~\ref{energy-gap}}, even though the state-of-the-art SR can greatly reduce energy consumption, a large gap ($\sim 20\%$) still exists when compared with the theoretical minimum energy consumption  



